QuRe: Query-Relevant Retrieval through Hard Negative Sampling in Composed Image Retrieval

Composed Image Retrieval (CIR) retrieves relevant images based on a reference image and accompanying text describing desired modifications. However, existing CIR methods only focus on retrieving the target image and disregard the relevance of other images. This limitation arises because most methods employing contrastive learning-which treats the target image as positive and all other images in the batch as negatives-can inadvertently include false negatives. This may result in retrieving irrelevant images, reducing user satisfaction even when the target image is retrieved. To address this issue, we propose Query-Relevant Retrieval through Hard Negative Sampling (QuRe), which optimizes a reward model objective to reduce false negatives. Additionally, we introduce a hard negative sampling strategy that selects images positioned between two steep drops in relevance scores following the target image, to effectively filter false negatives. In order to evaluate CIR models on their alignment with human satisfaction, we create Human-Preference FashionIQ (HP-FashionIQ), a new dataset that explicitly captures user preferences beyond target retrieval. Extensive experiments demonstrate that QuRe achieves state-of-the-art performance on FashionIQ and CIRR datasets while exhibiting the strongest alignment with human preferences on the HP-FashionIQ dataset. The source code is available at https://github.com/jackwaky/QuRe.

==> sections/07_Impact_Statement.tex <==
% \section{Impact Statement}

% This paper introduces \textbf{Qu}ery-\textbf{Re}levant Retrieval through Hard Negative Sampling~(\system{}), an approach to Composed Image Retrieval (CIR) that improves retrieval quality by retrieving both the target and other relevant images, improving user satisfaction. It addresses the false negative problem in CIR with a novel hard negative sampling strategy, advancing Machine Learning and Information Retrieval. \system{} contributes to improving search efficiency in e-commerce and visual search platforms, which benefits businesses and consumers by delivering more relevant search results. Additionally, the human preference-based evaluation (HP-FashionIQ dataset) aligns CIR models with human expectations, making AI-powered retrieval more user-centric.


==> tables/05_experiments/rerank_ablation.tex <==
\begin{table*}
\caption{Ablation study on defining the negative image set. (1) Baseline: The negative set is the whole candidate image corpus. (2) Top: The negative set is $n_{neg}$ images with the highest \system{} in the whole corpus for each query. \textbf{(3) Ours}: The negative set is $n_{neg}$ images with the highest \system{} in the set of images with a lower \system{} than the target image for each query.}
\centering
% \fontsize{6pt}{8pt}\selectfont
\renewcommand{\arraystretch}{1.2}
\footnotesize  % Reduce the font size
    \begin{tabular}{lcc|ccc}
    \toprule
    \multirow{1}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{CIRR}} & \multicolumn{3}{c}{\textbf{FashionIQ}}  \\ 
    \cmidrule(lr){2-3} \cmidrule(lr){4-6} 
     & R@5 + $\text{R}_s$@1 & Avg. & Avg R@10 & Avg R@50 & Avg. \\
    \midrule
    Baseline  & 75.96  & 81.46 & 52.22 & 73.51 & 62.86  \\
    Top & 80.96  & 84.52 & 52.92 & 73.87 & 63.39 \\
    \textbf{\system{}-Model} & \textbf{81.45}  & \textbf{84.92} & \textbf{54.89} & \textbf{74.97} & \textbf{64.93}   \\ 
    \bottomrule
    \label{table_ablation_rerank}
    \end{tabular}%
\end{table*}
\normalsize
